Model Reduction Using Sparse Polynomial Interpolation for the Incompressible Navier-Stokes Equations

This work investigates the use of sparse polynomial interpolation as a model order reduction method for the incompressible Navier-Stokes equations. Numerical results are presented underscoring the validity of sparse polynomial approximations and comparing with established reduced basis techniques. Two numerical models serve to access the accuracy of the reduced order models (ROMs), in particular parametric nonlinearities arising from curved geometries are investigated in detail. Besides the accuracy of the ROMs, other important features of the method are covered, such as offline-online splitting, run time and ease of implementation. The findings establish sparse polynomial interpolation as another instrument in the toolbox of methods for breaking the curse of dimensionality.

==> figures/tikz/l2_max_mean.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{semilogyaxis}[%
width=\fwidth,
height=\fheight,
at={(0.758in,0.481in)},
scale only axis,
xlabel={ \normalsize Reduced Dimension $n$ },
ylabel={ \normalsize Relative Error in Velocity },
xmin=0,
xmax=42,
ymin=0,
ymax=0.45,
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	0.401398274749373\\
2	0.311324706206876\\
3	0.128749798806262\\
4	0.128749798806262\\
5	0.0759163121561553\\
6	0.0489382287383231\\
7	0.0489382287383231\\
8	0.0247459506746621\\
9	0.0229354596945387\\
10	0.0163636938246672\\
11	0.0177976452071398\\
12	0.0153779236342024\\
13	0.0134205548368875\\
14	0.0138389464175648\\
15	0.0104124498450871\\
16	0.0104124498450871\\
17	0.00675615679272212\\
18	0.00640611557851343\\
19	0.0069675367629515\\
20	0.0069620370327461\\
21	0.00685580869062751\\
22	0.00685580869062751\\
23	0.00685580869062751\\
24	0.00239262424868225\\
25	0.00201693104329466\\
26	0.00204896853640157\\
27	0.00206315828768239\\
28	0.0019881255877119\\
29	0.00212389708000316\\
30	0.00161228045553771\\
31	0.00161228045553771\\
32	0.00119985389565971\\
33	0.0014036866979278\\
34	0.00138693515078041\\
35	0.00137857041783667\\
36	0.00134636894661437\\
37	0.00134636894661437\\
38	0.00134636894661437\\
39	0.00120041850790006\\
40	0.00120041850790006\\
41	0.0005518003872821\\
};
\addlegendentry{\normalsize Maximum $L^2$ error}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	0.209804601053099\\
2	0.168349126315326\\
3	0.0524343714539514\\
4	0.0541970051070021\\
5	0.040860556746052\\
6	0.0188158511769282\\
7	0.0190294455045341\\
8	0.0126373367933394\\
9	0.0114454871073537\\
10	0.00781063802012999\\
11	0.00817656820758803\\
12	0.00653582996440193\\
13	0.00557209518125903\\
14	0.00558359099767222\\
15	0.00305757735895357\\
16	0.0030188071032763\\
17	0.00189366997017362\\
18	0.00189850309814681\\
19	0.00179143453670143\\
20	0.00166753368425106\\
21	0.00140033855754212\\
22	0.00139287774066958\\
23	0.00136482144568802\\
24	0.000797760472455545\\
25	0.000770121845082735\\
26	0.000720704411037705\\
27	0.000744277552219612\\
28	0.000524587103735861\\
29	0.000527349716071102\\
30	0.000467602876424806\\
31	0.000433089467560394\\
32	0.00030284605918994\\
33	0.000294140235800106\\
34	0.000288934400390429\\
35	0.000262530609665316\\
36	0.000206190329039062\\
37	0.000206190329039062\\
38	0.000205631777131005\\
39	0.00014901290001233\\
40	0.000150645675356611\\
41	9.64945082298916e-05\\
};
\addlegendentry{\normalsize Mean $L^2$ error}

\end{semilogyaxis}


\end{tikzpicture}%

==> figures/tikz/pic1 <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{semilogyaxis}[%
width=\fwidth,
height=\fheight,
at={(0.772in,0.473in)},
scale only axis,
title ={\normalsize Comparison of standard RB method with sparse polynomial approximation},
xlabel={\normalsize Reduced Dimension $N$},
xmin=0,
xmax=18,
ylabel={\normalsize Relative $L^2$ Velocity Approximation Error},
ymin=0,
ymax=350,
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black},
legend style={at={(0.03,0.15)},anchor=west}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	0.818128693711737\\
2	0.519785949203545\\
3	0.23353665476975\\
4	0.0868583350087105\\
5	0.0286204802543573\\
6	0.00632740357089803\\
7	0.00240296141159437\\
8	0.000794381686006936\\
9	0.000401465640802809\\
10	0.000191336449572724\\
11	6.43378020415545e-05\\
12	3.07350787146857e-05\\
13	1.15575238113048e-05\\
14	4.8780290709573e-06\\
15	2.01563188522666e-06\\
16	8.98198061847425e-07\\
17	3.29628439717498e-07\\
};
\addlegendentry{mean error RB method}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	0.879789608787592\\
2	0.695035525860744\\
3	0.474156393530083\\
4	0.332216596213516\\
5	0.0595338643949694\\
6	0.0125148479311307\\
7	0.00438408010415915\\
8	0.00132762533603524\\
9	0.000687111432394074\\
10	0.000317493869600727\\
11	0.000108750451696693\\
12	5.45392145910203e-05\\
13	1.91374346491673e-05\\
14	8.3281905457113e-06\\
15	4.94946900551004e-06\\
16	3.55309329997724e-06\\
17	2.68967212359454e-06\\
};
\addlegendentry{max error RB method}

\addplot [color=mycolor3]
  table[row sep=crcr]{%
1	4.77790103758521\\
2	1.82930365876137\\
3	0.584725462337276\\
4	0.580562710544563\\
5	1.81448845861759\\
6	12.3641081034494\\
7	32.1512458085302\\
8	32.3789181538266\\
9	46.2080457169072\\
10	37.7319708070256\\
11	4.84919629471727\\
12	1.75817120529664\\
13	0.925884347515657\\
14	0.249549859395433\\
15	0.00801367103188836\\
16	0.00135028501757002\\
17	0.000692576030877893\\
};
\addlegendentry{mean error sparse polynomial approximation}

\addplot [color=mycolor4]
  table[row sep=crcr]{%
1	7.17832859195351\\
2	2.50077029214375\\
3	1.28367846202978\\
4	1.31443686352455\\
5	5.75826992607621\\
6	45.7082411097692\\
7	141.849103783939\\
8	179.765787142404\\
9	305.988581494307\\
10	302.890327396322\\
11	60.3545860604141\\
12	25.7059031917293\\
13	14.774329507544\\
14	4.47419766855062\\
15	0.155687789715775\\
16	0.0205953785411384\\
17	0.0192334431971036\\
};
\addlegendentry{max error sparse polynomial approximation}

\end{semilogyaxis}
\end{tikzpicture}%

==> figures/tikz/pic2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{semilogyaxis}[%
width=\fwidth,
height=\fheight,
at={(0.772in,0.473in)},
scale only axis,
xmin=0,
xmax=70,
title ={\normalsize Comparison of standard RB method with sparse polynomial approximation},
xlabel={\normalsize Reduced Dimension $N$},
ylabel={\normalsize Relative $L^2$ Velocity Approximation Error},
ymin=0,
ymax=1200,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black},
legend style={at={(0.15,.8)},anchor=west}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	0.818825272636841\\
2	0.519652934204976\\
3	0.234734775395549\\
4	0.0894169097166769\\
5	0.0290502744412072\\
6	0.00716784005663391\\
7	0.00264047500013066\\
8	0.00101363580412393\\
9	0.000479646371673897\\
10	0.00023488276492451\\
11	8.62885573476895e-05\\
12	3.8646658329785e-05\\
13	1.55456957228127e-05\\
14	6.22035209247412e-06\\
15	2.76180269383873e-06\\
16	1.13926568995396e-06\\
17	4.38740937195946e-07\\
18	2.09303681844716e-07\\
19	9.89436656883757e-08\\
20	6.51955117070142e-08\\
};
\addlegendentry{\normalsize mean error RB method}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	0.502835697017961\\
2	1.82930365876137\\
3	0.584725462337276\\
4	0.703727054164418\\
5	0.166336361274322\\
6	0.440925939508562\\
7	0.14095378346724\\
8	0.0355547466895943\\
9	0.0169035773759273\\
10	0.0866910307792859\\
11	0.0292654373198932\\
12	0.00950390802905611\\
13	0.0107802903697944\\
14	0.00390592183641382\\
15	0.00132489491736512\\
16	0.00964834144734535\\
17	0.00238322277841805\\
18	0.00138154231795551\\
19	0.000630844958143994\\
20	0.0023767905341087\\
21	0.000487624863493011\\
22	0.000234192476386166\\
23	0.000254839945012789\\
24	5.6647629288047e-05\\
25	3.40250831400077e-05\\
26	1.31279556968264e-05\\
27	8.31904170593274e-05\\
28	2.64307454307915e-05\\
29	2.8834299255837e-05\\
30	1.23423695872898e-05\\
31	6.88366842477314e-06\\
32	2.62282393997483e-06\\
33	1.19240542121488e-05\\
34	2.20100129208737e-06\\
35	7.91621720980402e-07\\
36	4.53008714860272e-07\\
37	1.77027753302006e-06\\
38	2.05861575824615e-06\\
39	4.15811017634727e-07\\
40	7.31943391709056e-07\\
41	2.26131082879867e-07\\
42	9.8741721187278e-08\\
43	2.62773168391321e-07\\
44	1.2085401608644e-07\\
45	5.53108973168817e-08\\
46	3.46483876994939e-07\\
47	1.61096399710646e-07\\
48	2.42353791753762e-07\\
49	7.8493683557287e-08\\
50	4.7616179219803e-08\\
51	5.32803677034863e-08\\
52	4.69412840037505e-08\\
53	6.15302486749242e-08\\
54	4.75987900083282e-08\\
55	1.33763199006206e-07\\
56	6.40421528059933e-08\\
57	4.60685804236036e-08\\
58	5.55435399960193e-08\\
59	4.74315077517778e-08\\
60	5.65756785975186e-08\\
61	4.15981759626415e-08\\
62	4.42366704048532e-08\\
63	4.0596519725701e-08\\
64	4.44031004487275e-08\\
65	4.09530930876115e-08\\
};
\addlegendentry{ \normalsize mean error Leja points}

\addplot [color=mycolor3]
  table[row sep=crcr]{%
1	0.289981905716959\\
2	0.141484017721139\\
3	0.584725420025328\\
4	0.703727032213992\\
5	0.157848582841308\\
6	0.417152294968255\\
7	0.119785805744536\\
8	0.0659685613827739\\
9	0.0157188225658593\\
10	0.0750899180717042\\
11	0.0244012815718787\\
12	0.0197021019288265\\
13	0.00442432948542695\\
14	0.00807823948899766\\
15	0.00172286513075547\\
16	0.000630105941732748\\
17	0.000302301809227888\\
18	0.00173790200609464\\
19	0.000564611387298806\\
20	0.0021034187265657\\
21	0.000528747988765063\\
22	0.000885168313989808\\
23	0.000165753607096798\\
24	0.000112536249166639\\
25	2.34752723985835e-05\\
26	0.000254328033847582\\
27	8.46003526593262e-05\\
28	0.00022834493410956\\
29	6.00943093414963e-05\\
30	2.21336560358004e-05\\
31	4.7920235703229e-06\\
32	5.53755131572251e-06\\
33	1.20123010619397e-06\\
34	7.10574706710264e-06\\
35	2.50883239791492e-06\\
36	1.09684092754157e-06\\
37	7.68585737839351e-07\\
38	2.42096724690971e-06\\
39	7.68620362072053e-07\\
40	1.21937824711655e-06\\
41	5.03504855467805e-07\\
42	1.63047957453824e-06\\
43	7.56914122347533e-07\\
44	7.02351212027397e-07\\
45	5.31131220115975e-07\\
46	1.77645618854243e-06\\
47	8.83445082460736e-07\\
48	1.59574871850362e-06\\
49	6.58351937711989e-07\\
50	6.25755671509312e-07\\
51	4.86183855268956e-07\\
52	5.08466863469673e-07\\
53	4.66450506921328e-07\\
54	5.83061049082908e-07\\
55	4.95417491776013e-07\\
56	5.5365506531451e-07\\
57	4.85844076349135e-07\\
58	4.81652048631058e-07\\
59	4.78608171969356e-07\\
60	5.06319292447481e-07\\
61	4.54789062532139e-07\\
62	6.69717253952861e-07\\
63	5.13807399159411e-07\\
64	5.2460954460516e-07\\
65	4.98727790207672e-07\\
};
\addlegendentry{\normalsize mean error symmetric Leja points}

\addplot [color=mycolor4]
  table[row sep=crcr]{%
1	0.502835693370456\\
2	1.82930352263811\\
3	0.584725420025328\\
4	0.6772127001627\\
5	0.16245584362802\\
6	0.428734271967916\\
7	0.137506639739893\\
8	0.0351095664884273\\
9	0.0169188717057015\\
10	0.0802907796448674\\
11	0.0270818562960138\\
12	0.00919880710709535\\
13	0.0100519319101257\\
14	0.00372407904784663\\
15	0.00128708243199118\\
16	0.00804573337734588\\
17	0.00198788967316274\\
18	0.00114382215995418\\
19	0.000492108611892055\\
20	0.00101510809152878\\
21	0.000205108033157792\\
22	0.000290355082318908\\
23	8.4873843884351e-05\\
24	0.000408348094746867\\
25	6.22752529441171e-05\\
26	2.65022801052285e-05\\
27	9.40830803547751e-06\\
28	3.56847397565597e-06\\
29	7.66419132212598e-06\\
30	3.50059592655859e-06\\
31	2.41541718857044e-06\\
32	8.29016019007718e-07\\
33	6.15312381563259e-07\\
34	5.89476443159158e-07\\
35	4.83550771645422e-07\\
36	4.75719010476425e-07\\
37	4.94427049098714e-07\\
38	6.31272461821226e-07\\
39	5.86878983074381e-07\\
40	6.20383859684885e-07\\
41	1.83761602788441e-06\\
42	1.98140770504473e-06\\
43	2.12372421386361e-06\\
44	4.37060640004323e-06\\
45	4.93539814064104e-06\\
46	8.18888580697652e-06\\
47	1.36232689535031e-05\\
48	1.25674263742469e-05\\
49	1.48681206723881e-05\\
50	3.68806740105581e-05\\
51	0.000134215383379285\\
52	0.000222053452343584\\
53	0.000463276773900247\\
54	0.00122907651449387\\
55	0.0102256615975448\\
56	0.0256764131407322\\
57	0.0544186828726237\\
58	1.33105513557723\\
59	2.20610903730362\\
60	8.81448209324827\\
61	17.1504349397231\\
62	86.8171127258625\\
63	153.750302143471\\
64	461.593171463953\\
65	1000.77352321406\\
};
\addlegendentry{\normalsize mean error equidistant points in Leja ordering}

\end{semilogyaxis}
\end{tikzpicture}%

==> figures/tikz/pic3.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}

\begin{semilogyaxis}[%
width=\fwidth,
height=\fheight,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=70,
title ={\normalsize Comparison of standard RB method with sparse polynomial approximation},
xlabel={\normalsize Reduced Dimension $N$},
ylabel={\normalsize Relative $L^2$ Velocity Approximation Error},
ymin=0,
ymax=40000,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black},
legend style={at={(0.15,.8)},anchor=west}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	0.8796936245888\\
2	0.69626269929828\\
3	0.480111523790192\\
4	0.339367792106783\\
5	0.0604178418979735\\
6	0.0144398634834675\\
7	0.00485398322570396\\
8	0.00174912061162311\\
9	0.000802039955153638\\
10	0.000392286591409484\\
11	0.000150857143184046\\
12	6.79590021403795e-05\\
13	2.5695064692032e-05\\
14	1.07473747635281e-05\\
15	6.38130859808699e-06\\
16	4.38907615469191e-06\\
17	3.36767688825056e-06\\
18	2.31797916520693e-06\\
19	1.96257197864325e-06\\
20	1.44818918971972e-06\\
};
\addlegendentry{\normalsize max error RB method}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	0.901026799634002\\
2	2.50077029214375\\
3	1.28367846202978\\
4	1.62252379462239\\
5	0.491817645757305\\
6	0.965070741637306\\
7	0.277481965507669\\
8	0.135365070427545\\
9	0.112046678928362\\
10	0.245716386662839\\
11	0.0669766988331191\\
12	0.051901136970085\\
13	0.0327108654666036\\
14	0.0146438247185773\\
15	0.00755094179030622\\
16	0.0287861143706663\\
17	0.0119163809514066\\
18	0.00844010896929804\\
19	0.00383608821991274\\
20	0.0079578657021794\\
21	0.00136874887133075\\
22	0.00106914999378585\\
23	0.000627756240344546\\
24	0.000238791034247058\\
25	0.000162430254023517\\
26	0.000138411274887118\\
27	0.000324732427145611\\
28	0.000265853807291145\\
29	0.000155036519835995\\
30	6.36917649747766e-05\\
31	2.43454881246988e-05\\
32	1.08366070846518e-05\\
33	4.69399597696269e-05\\
34	9.76284825450487e-06\\
35	4.61439127390537e-06\\
36	4.02294589301015e-06\\
37	5.82599434112924e-06\\
38	1.21311884117511e-05\\
39	2.52494500044002e-06\\
40	2.76139217909188e-06\\
41	4.46912066664576e-07\\
42	3.89272554331169e-07\\
43	7.11104172135643e-07\\
44	3.69452884680721e-07\\
45	3.69997814664589e-07\\
46	1.15263549639253e-06\\
47	4.77504313390003e-07\\
48	7.14775302308931e-07\\
49	3.62339706008897e-07\\
50	3.63127403366608e-07\\
51	3.66923818630454e-07\\
52	3.68144591090814e-07\\
53	3.62087039130865e-07\\
54	3.61538822150524e-07\\
55	5.161480298556e-07\\
56	3.74949050770419e-07\\
57	3.74065428517091e-07\\
58	3.66661607301082e-07\\
59	3.65815665521596e-07\\
60	3.58946441417279e-07\\
61	3.55795459546506e-07\\
62	3.52550118401449e-07\\
63	3.52576371181432e-07\\
64	3.50936049768198e-07\\
65	3.50013042775805e-07\\
};
\addlegendentry{\normalsize max error Leja points}

\addplot [color=mycolor3]
  table[row sep=crcr]{%
1	0.813004574281191\\
2	0.749339320265711\\
3	1.28367838011588\\
4	1.62252375053537\\
5	0.48812543530454\\
6	1.3123606846598\\
7	0.266236923736459\\
8	0.151643948870694\\
9	0.112137164168589\\
10	0.285592056798106\\
11	0.069261498850009\\
12	0.0590157675613906\\
13	0.0240741069636882\\
14	0.0458977268743702\\
15	0.00632096769464077\\
16	0.00513225273101653\\
17	0.00437126468527135\\
18	0.0103706935621418\\
19	0.00373714019551265\\
20	0.00936974665854293\\
21	0.0022786598479636\\
22	0.00276226792958801\\
23	0.000517546446780581\\
24	0.000368188843600977\\
25	0.000144558833638244\\
26	0.00143404812926275\\
27	0.000296761613954448\\
28	0.000808206458757501\\
29	0.000189095069253561\\
30	7.62989465251668e-05\\
31	1.7498729448289e-05\\
32	3.02177118534964e-05\\
33	4.69844442217186e-06\\
34	3.23656009017603e-05\\
35	7.01619278559439e-06\\
36	4.20762378017438e-06\\
37	3.25617563447814e-06\\
38	1.54416169568239e-05\\
39	2.63190448519917e-06\\
40	6.12371104724592e-06\\
41	2.31366533247325e-06\\
42	5.00272526922262e-06\\
43	2.57457145060176e-06\\
44	2.52320639980971e-06\\
45	2.51320572584348e-06\\
46	6.97047981511792e-06\\
47	2.98968667056013e-06\\
48	5.91303311047568e-06\\
49	2.49384044285118e-06\\
50	2.39948443128564e-06\\
51	2.39501733272412e-06\\
52	2.40031868336498e-06\\
53	2.40023438452766e-06\\
54	2.4273525389565e-06\\
55	2.41678003117269e-06\\
56	2.41558700050709e-06\\
57	2.41773307581811e-06\\
58	2.45281800044606e-06\\
59	2.49654753998829e-06\\
60	2.33067909339259e-06\\
61	2.33269440171978e-06\\
62	2.98327546899736e-06\\
63	2.96501736606224e-06\\
64	2.94840149135017e-06\\
65	2.94907970430462e-06\\
};
\addlegendentry{\normalsize max error symmetric Leja points}

\addplot [color=mycolor4]
  table[row sep=crcr]{%
1	0.901026797608989\\
2	2.50077010721653\\
3	1.28367838011588\\
4	1.55619930972249\\
5	0.503888200731958\\
6	0.937288053778587\\
7	0.261529843166728\\
8	0.133509566599905\\
9	0.110789556852393\\
10	0.214890770284976\\
11	0.0717620276156125\\
12	0.0554964545629058\\
13	0.0284281645227232\\
14	0.013915684655235\\
15	0.0060333665693543\\
16	0.024190633478345\\
17	0.00926618699802463\\
18	0.00654366432953591\\
19	0.00243380019082687\\
20	0.00360941944472201\\
21	0.000844778322300081\\
22	0.000754932021064886\\
23	0.000458767970286524\\
24	0.00110475541447264\\
25	0.000204384023808726\\
26	0.000104120817186126\\
27	2.05720975886559e-05\\
28	1.81789951414047e-05\\
29	2.45456064255324e-05\\
30	1.3436020685058e-05\\
31	8.38381386374508e-06\\
32	3.92439134979546e-06\\
33	3.63412857949954e-06\\
34	2.56678324467091e-06\\
35	2.50434030933546e-06\\
36	2.47117549015588e-06\\
37	2.94372212943247e-06\\
38	3.16779614255939e-06\\
39	3.96269507683927e-06\\
40	5.16652877533434e-06\\
41	4.21253511124659e-05\\
42	5.24537828683835e-05\\
43	5.91594958098867e-05\\
44	0.000141610870723541\\
45	0.000163635965862259\\
46	0.00028579080736356\\
47	0.000490490055135749\\
48	0.000451153418784304\\
49	0.000539784446453142\\
50	0.00138236301348867\\
51	0.00509509905518118\\
52	0.00847407970717039\\
53	0.017808272403902\\
54	0.0473509593182651\\
55	0.394904459196678\\
56	0.993488965305378\\
57	2.10914586186018\\
58	51.7171908723806\\
59	85.8073246630279\\
60	343.493334615912\\
61	669.092263188861\\
62	3393.12882478381\\
63	6014.58352959697\\
64	18081.4622411107\\
65	39241.2479817766\\
};
\addlegendentry{\normalsize max error equidistant points in Leja ordering}

\end{semilogyaxis}
\end{tikzpicture}%
